AutoCorrect: Deep Inductive Alignment of Noisy Geometric Annotations

We propose AutoCorrect, a method to automatically learn object-annotation alignments from a dataset with annotations affected by geometric noise. The method is based on a consistency loss that enables deep neural networks to be trained, given only noisy annotations as input, to correct the annotations. When some noise-free annotations are available, we show that the consistency loss reduces to a stricter self-supervised loss. We also show that the method can implicitly leverage object symmetries to reduce the ambiguity arising in correcting noisy annotations. When multiple object-annotation pairs are present in an image, we introduce a spatial memory map that allows the network to correct annotations sequentially, one at a time, while accounting for all other annotations in the image and corrections performed so far. Through ablation, we show the benefit of these contributions, demonstrating excellent results on geo-spatial imagery. Specifically, we show results using a new Railway tracks dataset as well as the public INRIA Buildings benchmarks, achieving new state-of-the-art results for the latter.

==> fig_tab/Fig-align_curves.tex <==
\begin{table}[t]
\centering
\includegraphics[width=.6\textwidth]{figure/inria_align}
\captionof{figure}{Building alignment result. 
We outperform all recent works at all thresholds, 
especially when the threshold approaches around 10 pixels, our accuracy achieve almost $100\%$.}\label{Fig.align_result}
\end{table}

==> fig_tab/Fig-fail.tex <==
\begin{figure*}[!htb]
\centering
\tabcolsep=0.02cm
\renewcommand{\arraystretch}{0.25}
\begin{tabular}{
  >{\centering\arraybackslash} m{0.23\textwidth}
  >{\centering\arraybackslash} m{0.23\textwidth}
  >{\centering\arraybackslash} m{0.23\textwidth}
  >{\centering\arraybackslash} m{0.23\textwidth}}      
\includegraphics[width=1\linewidth]{figure/rail_fail1} &
\includegraphics[width=1\linewidth]{figure/rail_fail2} &
\includegraphics[width=1\linewidth]{figure/im_1_01848_00924} &
\includegraphics[width=1\linewidth]{figure/im_1_01617_00000}\\
\end{tabular}
\vspace{-1em}
\caption{Failure cases. Invisiable objects (railways, buildings) on satellite image causes the inaccurate predictions.
}\label{fig.failure_case}
\end{figure*}

==> sec/Proposed_method_az.tex <==
\section{Approach}
\label{Map Feature Extraction}

Our goal is to train deep networks for the detection of visual objects while relying on noisy labels.
While the approach is fairly general, we apply it to the detection of objects such as building and roads in geo-spatial images, where noisy labels can be extracted from on-line data repositories such as mapping services.
The mismatch between annotations and images is sometimes large, as shown in \cref{Fig.data}.
Na\"\i{}vely training a model with these annotations leads to inaccurate predictions.


\input{fig_tab/Fig-consistency}

There are two main challenges. First, all annotations are potentially noisy and thus it is not clear how the noise can be identified and removed.
Second, as different objects in the image may be misaligned in different ways, we must enable instance-level corrections while handling an arbitrary number of object instances per image.
We address these challenges in three ways.
First, we use a self-supervised consistency loss based on the fact that multiple perturbations of the same label must always map to the same noiseless label.
Second, we show that the intrinsic symmetry of certain visual objects provides a powerful implicit constraint that can reduce the ambiguity in the annotation clean-up process.
Third, we introduce the idea of inductive alignment, adjusting labels one instance at a time, sequentially, keeping track of the algorithm state by means of a \emph{spatial memory map}.
This is implemented by a recurrent neural network (RNN), which applies the same alignment logic to each annotation, but accounting for annotations already processed.

\subsection{Single instance alignment}\label{s:single}

We start by describing a neural network architecture that can predict a translation and rotation for an individual object annotation in order to better align it to the image content. 
Note that, while this task may sound similar to object detection, it is in fact much easier as the annotation cues us to the \emph{existence} and rough location of an object.

At each step, the input to the model is a concatenation of the RGB image $I\in\mathbb{R}^{3\times H\times W}$ with a scalar label map $y\in\{0,1\}^{H\times W}$ which encodes the annotation as a binary image.
We know that the annotations can potentially be noisy, so we wish to learn a predictor function that outputs the transformation to align the image and annotation.
This is implemented using a CNN that takes as input $I$ and $y$ and outputs a transformation $t$:
\begin{align}\label{e:model}
t = \Phi(I,y).
\end{align}
The corrected annotation $\hat{y} = t \cdot y$ is expressed as the transformed version of the annotation $y$ by the predicted transformation $t \in G$, where $G$ is a group of transformations $\mathbb{R}^2\rightarrow\mathbb{R}^2$ such as 2D similarities.
The symbol $\cdot$ denotes warping an image by a transformation.

% If the annotation is noise-free, $t$ is expected to be an identity matrix and $\hat{\mathbf{y}} = \mathbf{y}$. If the annotation is noisy, 
% the corrected annotation $\hat{\mathbf{y}}$ should approximate the underlying noise-free annotation $\mathbf{y}_{\text{gt}}$, which however is never observed during training.

%\subsubsection{Geometry}\label{s:geom}

Model~\eqref{e:model} has several useful geometric properties:
\begin{lemma}\label{l:one}
If $y_\text{gt}$ is the ground-truth annotation for image $I$, then
$
\Phi(I,y_\text{gt})= 1
$
is the identity transformation. Furthermore, for all invertible transformations $g \in G$, we have
$
\phi(g\cdot I,y) = g \Phi(I,y)
$
and
$
\phi(I,g\cdot y) = \Phi(I,y) g^{-1}.
$
\end{lemma}
The lemma is easy to prove once we note that, if $y_\text{gt}$ is the ground-truth label of image $I$, then $g \cdot y_\text{gt}$ is the ground-truth label of image $g \cdot I$.
From this lemma, we can also see that any annotation that can be recovered from an image must have the same \emph{symmetries} as the image itself:

\begin{lemma}
Let $\hat{y} = \Phi(I,y) \cdot y$ be the annotation reconstructed from image $I$ using model~\eqref{e:model} and assume that $m\in G$ is a symmetry of the image, \ie $I = m \cdot I$.
Then the reconstructed annotation has the same symmetry, in the sense that $\hat{y} = m \cdot\hat{y}$.
\end{lemma}

\begin{proof}%
\hfill %
$
\hat{y}
= \Phi(I,y) \cdot y
= \Phi(m\cdot I,y) \cdot y 
= m \Phi(I,y) \cdot y
= m  \cdot \hat{y}.
$\hfill%
\end{proof}

This lemma shows that annotations can be predicted from images only if they have the same symmetries as the images.
For example, if the model labels a straight road with a line, then the line must coincide to the road axis of symmetry.
Hence image symmetries implicitly constrain the predictor~\eqref{e:model} (in the example of the road, the correction must move the line onto the visual axis of symmetry of the road), reducing the ambiguity in registering the annotation.
Note that this effect does not require specific images to be exactly symmetric; rather, it suffices that the object category is \emph{statistically} symmetric (for example it is not possible to tell the direction of a road even if there are a few trees on one side, making the image asymmetric).

%\subsubsection{Self-supervised learning}\label{s:self}

If we assume all labels are correct, \ie $y = y_{gt}$, 
then \cref{l:one} can be used to train model~\eqref{e:model} via self-supervised learning.
The idea is to perturb the noise-free annotations synthetically by applying a random transformation $g \in G$ to the annotation $y = y_\text{gt}$.
From~\cref{l:one}, and using the assumption $y = y_\text{gt}$, we have
$
\Phi(I, g \cdot y) = \Phi(I,y) g^{-1} = 1 g^{-1} = g^{-1}.
$
We may capture this constrain in the {\em self-supervised loss}:
\begin{equation}\label{e:loss1}
J_1 = \|g^{-1} - \Phi(I, g\cdot y)\|^2
\end{equation}
However, in our case $y_{gt}$ is unknown so this loss can be used only as an approximation.
In this case, the constraint can be written in term of \emph{relative} transformations.
To this end, consider applying two random transformations $y_1 = g_1 \cdot y$ and $y_2 = g_2 \cdot y$ to the annotation $y$.
From~\cref{l:one}, we have
$
\Phi(I,g_1\cdot y) g_1 = \Phi(I,y)  = \Phi(I,g_2\cdot y) g_2.
$
This can be written as a {\em consistency loss}:
\begin{equation}\label{e:loss2}
J_2 = \|t_1 g_1 - t_2 g_2\|^2,
\quad
t_1 = \Phi(I,g_1\cdot y),
\quad
t_2 = \Phi(I,g_2\cdot y).
\end{equation}
% as there exists an unknown transformation between the ground-truth and provided annotation, \ie $y_{gt} = h \cdoty$, $h\in G$.
% To cope with this situation, we apply a transformation consistency loss.
% For an image-label pair $(I,y)$, 
% assume two random transformations are applied to the annotation, \ie $y_1 = g_1 y$ and $\boldsymbol{y}_2 = g_2 y$.
% When passing the image and annotation for alignment, 
% we get $\hat{g}_1 = \Phi(I, y_1)$, $\hat{g}_2 = \Phi(I, y_2)$.
% Note that, for noisy annotations, $\hat{g}_1 \neq g^{-1}_1$, $\hat{g}_2 \neq g^{-1}_2$,
% but we should expect to minimize the objective function defined as:
% \begin{align}
% J_2 = ||\hat{g}_1 \cdot g_1 - \hat{g}_2 \cdot g_2||^2.
% \end{align}
Intuitively, when two random transformations operate on the annotation, an ideal alignment model should be able to transform the annotation back to the same position, as $y_{gt}$ is unique.

Overall, to train the model on noisy data, we therefore consider a weighed combination $J = \alpha_1 \cdot J_1 + \alpha_2 \cdot J_2$ (details in \cref{sec:training}).
% \begin{equation}\label{e:joint}
% J = \alpha_1 \cdot J_1 + \alpha_2 \cdot J_2.
% \end{equation}

\subsection{Inductive alignment}\label{regress}

\input{fig_tab/Fig-net}

A na\"\i{}ve implementation of model~\eqref{e:model} may align single object instances well, but it would fail when an image contains multiple object occurrences, especially when, as in satellite images, these are spatially close and similar in appearance.
In particular, independent alignment may cause different noisy annotations to be incorrectly associated to the same object occurrence.
To tackle this challenge, we introduce an inductive alignment model which uses an external \emph{spatial memory map} to make the algorithm aware of all annotations present in the image as well as to keep track of all correction processed so far.
% However, labels could be noisy, we therefore update the \emph{spatial memory map} with our predictions.
% Given the network that can align single object instance independently, 
% we move to the problem of aligning \emph{all} the annotations ($y = \{y_i\}_{i=1}^{n}$) in an image.
% The challenges are therefore two-fold:
% Firstly,  an ideal model should focus its attention to one object at a time, 
% while being aware of the allocations already performed,
% such that multiple object labels are not associated to the same location.
% Secondly, the proposed approach should be able to generalize to arbitrary number of instances during test time. 
% We achieve this by introducing a model for inductive alignment,
% specifically, 
% we propose an external \emph{spatial memory map} to keep a tab on the objects that have been processed so far,
% and therefore the current alignment step conditions on all other instances.
Formally, given a training image $I$ with $n$ object annotations $\mathbf{y}=(y_1,\dots,y_n)$, our goal can be seen as estimating the joint posterior density of the transformation matrix for all the noisy object annotations~$p({\{t_i\}}_{i=1}^{n}|I, \mathbf{y})$.
Rather than modelling multiple object annotations simultaneously, we break this down as \emph{sequence} of simpler steps, in which a single transformation is predicted at a time, conditioned on the previous decisions, resembling an autoregressive model.
Formally, this autoregressive model can be written as:
$
P(t_1, t_2, \ldots, t_n| I, \mathbf{y}) =
P(t_1 | I, \mathbf{y})
P(t_2 | I, t_1, \mathbf{y})
\cdots
P(t_n | I, \{t_i\}_{i=1}^{n-1},\mathbf{y}).
$
Note that this process requires learning a sequence of models $P(t_i | I, t_1,\dots,t_{i-1}, \mathbf{y})$.
Directly parameterising the relations among transformations is difficult and results in a model which is rather opaque;
instead, we propose to summarise the effect of conditioning on the previous corrections $t_1,\dots,t_{i-1}$ via a \emph{spatial memory map} $M_{i-1}$, 
ideally, the memory map should represent all annotations and 
corrections performed so far \emph{except} the annotation $y_i$ that is currently being processed,

** I think it would be better to give the explicit example first, and then to write this more formally as an induction
algorithm, i.e. give the starting state, and then the update step and termination **

formally:
\begin{equation}
P(t_i |I, t_1,\dots,t_{i-1},\mathbf{y})=P(t_i |I,M_{i-1},y_i), \qquad
M_i = M_{i-1} + t_{i} \cdot y_{i} - y_{i+1}.
\end{equation}

Expanding the recurrence above, 
this is given by $M_i = \sum_{j=1}^{i} t_j \cdot y_j + \sum_{j=i+2}^n y_j$ where $M_0 = y_2 + \cdots + y_n$.

An explicit example is illustrated in~\cref{Fig.net}, showing four railway track annotations to be corrected.
At the very first step, 
the algorithm starts with four binary masks, each coding one of the noisy railway annotations. 
All annotations but the first are summarised in the memory $M$, 
and the first annotation is concatenated as an additional input~($y_1$)  to the network $\Phi$.
Then, the first annotation $y_1$ is corrected by predicting the rigid transformation $t_1$, 
and the memory $M$ is updated by adding the image of $t_1 \cdot y_1$ and removing the image of annotation $y_2$, 
readying for the next cycle.

\subsection{Implementation details}
\label{sec:training}

Consider a training image $I$ with $n$ noisy object annotations $\mathbf{y}=(y_1,\dots,y_n)$.
Annotations are perturbed by applying random transformations $g \cdot y_i$ where $g$ is the composition of a translation of up to $25$px in each direction and a rotation of up to 5 degrees (clockwise or anticlockwise) as this was found to be commensurate to the maximum amount of noise in the geo-spatial datasets we used for assessment.

During early training, we set the gating parameters in the joint objective function $J$ as $\alpha_1 = \alpha_2 = 1$.
This ensures the model converges quickly to an approximate solution within a few pixels of the ground-truth annotation despite the fact that all annotations are noisy so that term $J_1$ in the objective function is not exactly valid.
In a second phase, when the model is close to the final solution, the terms $J_1$ and $J_2$ start to be in conflict for the annotations that contain the largest amount of noise.
Hence the coefficient $\alpha_1$ and $\alpha_2$ are adjusted as follows:
\begin{align}\label{equation_gating}
\begin{cases}
\alpha_1 =0,~\alpha_2 =1 & \text{if
$
\min(
\operatorname{IoU}(t_1 g_1 \cdot y,y), 
\operatorname{IoU}(t_2 g_2 \cdot y,y)) < 0.2
$
},  \\
\alpha_1 =1,~\alpha_2 =0 & \text{otherwise},\\
\end{cases}
\end{align}
where $\operatorname{IoU}$ denotes the standard \emph{Intersection over Union} measure.
This states that when any of the predicted corrections are far away from the given label, the label is expected to contain a large amount of noise, only the consistency loss $J_2$ is applied; otherwise only the stricter self-supervised loss $J_1$ is used.

\paragraph{Architecture and optimisation.}

The proposed \emph{learn-to-align} model uses as backbone architecture the VGG-M network~\cite{Chatfield14} with minor modifications (details in the supp.~mat.).
The network is trained using the Adam optimiser at an initial learning rate of $10^{-4}$, which is divided by $10$ after the training error plateaus.

